EtherSolve: Computing an Accurate Control-Flow Graph from Ethereum Bytecode

Motivated by the immutable nature of Ethereum smart contracts and of their transactions, quite many approaches have been proposed to detect defects and security problems before smart contracts become persistent in the blockchain and they are granted control on substantial financial value. Because smart contracts source code might not be available, static analysis approaches mostly face the challenge of analysing compiled Ethereum bytecode, that is available directly from the official blockchain. However, due to the intrinsic complexity of Ethereum bytecode (especially in jump resolution), static analysis encounters significant obstacles that reduce the accuracy of exiting automated tools. This paper presents a novel static analysis algorithm based on the symbolic execution of the Ethereum operand stack that allows us to resolve jumps in Ethereum bytecode and to construct an accurate control-flow graph (CFG) of the compiled smart contracts. EtherSolve is a prototype implementation of our approach. Experimental results on a significant set of real world Ethereum smart contracts show that EtherSolve improves the accuracy of the execrated CFGs with respect to the state of the art available approaches. Many static analysis techniques are based on the CFG representation of the code and would therefore benefit from the accurate extraction of the CFG. For example, we implemented a simple extension of EtherSolve that allows to detect instances of the re-entrancy vulnerability.

==> precision_recall_old.tex <==
\subsection{Precision and Recall}
\label{ssec:precision-recall}

% 1- cosa sono precision and recall in relazione al nostro progretto? precision corrisponde alla relazione tra le funzioni ...
% 2- riportare (sistemare schema insiemistico significativo precision and recall)
% 3- riportare due formule di precision recall (livello di dettaglio?)
% 4- riflessioni sui risultati sia per singoli contratti specifici che in generale (media di tutte le precision e recall)
% 6- errori di identificazione delle funzioni? il dispatcher è sufficiente a determinare quali sono le funzioni e a ricostruire l'ABI
% 7- Sottolineare che tale misura non copre l'intero CFG ma solamente la parte iniziale, in particolare il dispatcher
% 8- Giustificare il fatto che se la precision e la recall siano alte e dunque sono state rilevate molte funzioni correttamente allora probabilmente il contratto è stato ricostruito correttamente a  livello di CFG (saltrimenti facciamo precision e recall alla cazzo)

% Precision recall: 0,98829257356079	0,986431847390076

To evaluate the effectiveness of the tool we chose the standard method of precision and recall. %, and we modeled it in three differents ways to consider increasingly stringent specifications.
The aim of this phase is to check how well the tool is able to identify the functions of the Solidity contract from the CFG, comparing them with those declared in the contract ABI.



Once the hashes are extracted, \ethersolve{} downloads and analyses the contract ABI, computing the signatures and the hashes of the functions and then proceeds with the comparison, calculating the precision and the recall for each contract.


The tool manages to correctly build the CFG and extract the hashes for 996 contracts among the 1000 in the dataset, due to internal errors in some particular cases. For the correctly analysed CFGs the average values for precision and recall are respectively $0.988$ and $0.986$, considering that the average functions number in each contract is 19.

% \begin{figure}
%     \centering
%     \begin{tikzpicture}
%         \filldraw [fill=black!10!white, draw=black] (-2,-2) rectangle (2,2);
%         \filldraw [fill=black!20!white, draw=black] (0,0) circle (1.5cm);
%         %\draw [] (-2,-2) -- (2,2);
%         \node [align=left] at (-1,1.75) {$F_N$ \par};
%         \node [align=left] at (-0.5,0.5) {$T_P$\par};
%         \node [align=left] at (0.5,-0.5) {$F_P$ \par};
%         \node [align=left] at (1,-1.75) {$T_N$ \par};
%         % points1
%         \filldraw [] (0,1) circle (1pt);
%         \filldraw [] (-1,0.25) circle (1pt);
%         \filldraw [] (-0.75,-0.4) circle (1pt);
%         \filldraw [] (-1.5,1.25) circle (1pt);
%         \filldraw [] (0.5,1.75) circle (1pt);
%         \filldraw [] (-1.75,-0.5) circle (1pt);
%         % points2
%         \draw [] (0,-1) circle (1.5pt);
%         \draw [] (1,-0.25) circle (1.5pt);
%         \draw [] (0.75,0.4) circle (1.5pt);
%         \draw [] (1.5,-1.25) circle (1.5pt);
%         \draw [] (-0.5,-1.75) circle (1.5pt);
%         \draw [] (1.75,0.5) circle (1.5pt);
%         % Legenda
%         \filldraw [] (3,0.5) circle (1pt);
%         \node [align=left] at (3.75,0.5) {$\in H_A$};
%         \draw [] (3,0) circle (1.5pt);
%         \node [align=left] at (3.75,0) {$\notin H_A$};
%         \filldraw [fill=black!20!white] (3,-0.5) circle (4pt);
%         \node [align=left] at (3.75,-0.5) {$= H$};
%     \end{tikzpicture}
%     \caption{Precision e Recall}
%     \label{fig:precision-recall}
% \end{figure}
